Watching the IPv6 Takeoff from an IXP's Viewpoint

The different level of interest in deploying the new Internet address space across network operators has kept IPv6 tardy in its deployment. However, since the last block of IPv4 addresses has been assigned, Internet communities took the concern of the address space scarcity seriously and started to move forward actively. After the successful IPv6 test on 8 June, 2011 (World IPv6 Day [1]), network operators and service/content providers were brought together for preparing the next step of the IPv6 global deployment (World IPv6 Launch on 6 June, 2012 [2]). The main purpose of the event was to permanently enable their IPv6 connectivity. In this paper, based on the Internet traffic collected from a large European Internet Exchange Point (IXP), we present the status of IPv6 traffic mainly focusing on the periods of the two global IPv6 events. Our results show that IPv6 traffic is responsible for a small fraction such as 0.5 % of the total traffic in the peak period. Nevertheless, we are positively impressed by the facts that the increase of IPv6 traffic/prefixes shows a steep increase and that the application mix of IPv6 traffic starts to imitate the one of IPv4-dominated Internet.

==> background.tex <==
\section{History and Background}
\label{sec:background}



